Measuring the Cosmic X-ray Background in 3-20keV with Straylight from NuSTAR

By characterizing the contribution of stray light to large datasets from the NuSTAR X-ray observatory collected over 2012--2017, we report a measurement of the cosmic X-ray background in the 3--20 keV energy range. These data represent $\sim20\%$ sky coverage while avoiding Galactic Ridge X-ray emission and are less weighted by deep, survey fields than previous measurements with NuSTAR. Images in narrow energy bands are stacked in detector space and spatially fit with a model representing the stray light and uniform pattern expected from the cosmic X-ray background and the instrumental background, respectively. We establish baseline flux values from Earth-occulted data and validate the fitting method on stray light observations of the Crab, which further serve to calibrate the resulting spectra. We present independent spectra of the cosmic X-ray background with the FPMA and FPMB detector arrays, which are in excellent agreement with the canonical characterization by HEAO 1 and are $10\%$ lower than most subsequent measurements; $F_{\rm{3-20~keV}}^{FPMA} = 2.63 \times 10^{-11}~\rm{erg~s^{-1}~cm^{-2}~deg^{-2}}$ and $F_{\rm{3-20~keV}}^{FPMB} = 2.58 \times 10^{-11}~\rm{erg~s^{-1}~cm^{-2}~deg^{-2}}$. We discuss these results in light of previous measurements of the cosmic X-ray background and consider the impact of systematic uncertainties on our spectra.

==> obslistforpaper.tex <==
60001113002     255.31   51.80    76.76    76.75    23.39    23.38
30002039003     229.03   56.27    67.88    67.81     3.96     3.95
30001004004     224.63   -31.65    60.85    60.83    28.56    28.52
60110003003     189.13   62.20    59.72    59.56    15.77    15.92
60110003004     189.16   62.20    60.18    59.97    13.75    13.71
60001107002     156.62   25.73    59.10    59.05    22.93    22.92
60110002004     189.23   62.23    57.20    57.40    13.02    13.08
60110001003     189.28   62.28    55.04    55.00    17.73    17.68
60101004002     328.74   -9.40    53.89    53.58    13.51    13.46
60110001005     189.31   62.27    53.77    53.85    10.41    10.38
60001136002     190.87   -2.54    50.75    50.97     9.07     9.06
60366002002     352.63   -0.65    50.84    50.46    17.94    17.86
60110003005     189.16   62.19    49.61    49.57    21.10    21.06
60110001007     189.31   62.27    48.27    48.71    20.87    21.01
60110002005     189.24   62.23    48.60    48.68    20.90    20.84
60110003002     189.20   62.20    42.31    42.11    18.85    18.81
60110002001     189.28   62.24    41.92    41.84    18.87    19.02
60110001001     189.35   62.28    42.58    42.38    18.96    18.92
60362025002     324.81   -26.76    42.28    41.85    11.78    11.54
60101084002     178.04   -0.76    41.35    41.28     5.30     5.29
60201019002     181.07   19.40    40.70    40.81    11.11    11.11
60101083002     218.77   -1.73    41.10    40.72    11.83    11.70
90361003004     197.40   -23.39    39.04    38.85     4.41     4.50
60201017002     145.30   34.73    37.56    37.09     3.82     3.71
60001156004     159.24   4.85    35.78    35.72     6.45     6.44
60001123002     194.23   4.46    28.75    28.93     8.82     8.81
60001150002     165.11   29.00    27.83    27.79    12.22    12.21
60101073002     181.67   -31.94    27.69    27.45     2.22     2.22
60001120002     121.12   65.00    27.50    27.38     8.47     8.47
60101065002     183.80   -14.50    26.48    26.46     2.97     2.96
60361023002     233.87   73.46    26.31    26.51    10.14    10.40
60101082002     196.27   0.91    26.14    26.25     6.13     6.13
50101005002     175.44   32.28    26.44    25.91     3.65     3.64
60101064002     182.41   -5.03    25.09    25.07     4.97     5.08
60001121002     211.20   43.44    25.70    25.68     0.01     0.01
60001141004     5.52   -18.93    24.18    24.15     6.12     6.11
60001092002     220.27   -37.07    23.99    23.75    10.42    10.21
90361003002     197.40   -23.39    23.21    23.26     3.42     3.32
60001061002     14.08   0.51    21.57    21.53     4.70     4.70
60001071002     179.37   60.05    21.44    21.41     4.67     4.67
60001114002     273.57   34.17    21.06    21.02     4.87     4.85
60001115002     331.91   19.63    20.51    20.48     8.88     8.87
60001069002     145.15   3.56    20.38    20.44     7.13     7.19
60001119002     11.46   4.20    19.80    19.76    11.84    11.81
60101072002     151.05   -6.46    19.36    19.51     5.13     5.06
60001122002     151.06   5.22    19.34    19.21     2.81     2.80
90361003006     197.41   -23.39    18.84    18.91     1.09     1.09
60001065002     2.79   0.91    17.99    17.97     2.30     2.29
90361015002     199.92   -27.42    11.60    11.58     1.93     1.92
90361002002     194.33   -19.69     8.88     8.85     0.76     0.72
60023005003     214.92   52.89    48.73    48.59    21.43    21.46
60023007003     215.13   53.04    50.07    49.95    21.52    21.40
60110002003     189.20   62.24    61.90    61.82    17.76    17.81
50101003002     214.74   21.05    81.91    82.31    15.00    14.96
60001141002     5.52   -18.93    81.78    83.26    23.02    23.03
60101040002     278.90   43.90   149.00   149.08    12.04    11.94
60021001002     149.75   2.47    21.70    21.76     9.72     9.61
60023002002     214.63   52.63    48.45    48.23     4.19     4.18
60023002003     214.59   52.66    46.19    46.09    21.71    21.67
60021062001     149.93   1.86    24.07    23.86     8.86     8.85
60001165002     313.13   9.86    29.12    29.08     5.09     5.08
60021005001     149.72   2.04    22.46    22.45    10.62    10.61
60021006001     149.71   1.93    24.76    24.72    10.41    10.39
60021096001     150.12   1.68    27.14    27.19    12.60    12.58
60021007001     149.86   2.46    23.23    23.20     9.92     9.92
10060004002     238.88   -33.23    30.48    30.54    10.56    10.38
60101048002     49.02   -2.39    50.30    49.86    10.66    10.52
60021011001     149.82   2.03    26.97    27.14    11.83    11.92
60111001002     34.09   -5.20    47.18    47.28    15.56    15.81
60021012001     149.81   1.92    25.85    26.01    10.28    10.26
60111041001     34.44   -4.83    50.54    50.27    24.29    24.33
60021107001     150.68   1.97    30.32    30.37    13.97    13.95
60021094001     149.90   1.70    26.96    26.81    12.43    12.41
60111012001     34.37   -5.23    48.83    48.22     9.98    10.03
60111019002     34.52   -5.09    51.20    51.08     7.13     7.02
60101071002     144.21   48.47    20.70    20.52     2.29     2.28
60001090002     164.79   24.53    24.35    24.01    10.40    10.28
60021063001     149.82   1.87    24.97    24.95     7.31     7.39
60111044001     34.25   -4.90    50.87    50.81    23.56    23.51
60111037001     34.74   -4.93    49.93    49.81    24.20    24.14
60021067001     150.54   2.74    26.17    26.10    11.41    11.38
60021100001     150.54   1.65    27.23    27.26    12.59    12.57
60022015003     53.18   -27.62    47.54    47.32     8.59     8.68
60101069002     4.71   -10.41    20.15    20.20    10.01     9.99
60001156006     159.21   4.85    20.75    20.91     9.51     9.41
30002039002     229.06   56.27    44.89    44.69     0.02     0.02
60021089001     149.59   1.94    26.25    26.29    11.94    12.01
60001132002     130.13   38.60    46.77    46.62    14.22    14.18
10060002002     90.50   -86.43    16.96    16.93     6.75     6.74
60111009002     34.31   -5.15    47.75    47.43    11.23    11.09
60022014001     53.05   -27.64    48.80    48.85    22.18    22.26
60001124002     147.44   29.93    34.63    34.58     8.37     8.36
60021104001     150.57   1.87    26.81    26.76    12.61    12.59
60021075001     149.98   2.68    27.23    27.47    12.20    12.19
60111007002     34.24   -5.07    47.06    47.66    11.91    12.26
60021014001     149.96   2.35    24.12    24.10    10.65    10.65
60021054001     150.32   2.59    17.96    17.93     9.58     9.57
60021117001     150.72   2.53    26.71    26.66    12.90    12.88
60023002004     214.58   52.64    51.81    51.61    11.04    11.05
60023002005     214.62   52.63    51.85    51.59     3.80     3.80
60023005004     214.90   52.86    49.83    49.63     6.92     6.91
60023005001     214.95   52.86    50.01    50.02     5.85     5.84
60022006002     53.06   -27.84    45.09    44.97     5.32     5.13
60021071001     150.21   2.66    26.33    26.47     9.80     9.88
60021015001     149.95   2.24    26.64    26.60    10.43    10.41
60021025001     150.19   2.44    25.11    24.98    11.06    10.85
60111003002     34.16   -5.14    48.10    48.44    14.56    14.80
60023006004     215.01   52.94    48.02    48.08     6.59     6.58
60023006002     215.05   52.93    50.41    51.07     7.11     7.10
60023006003     215.02   52.97    49.39    49.43    21.20    21.35
60021087001     149.61   2.16    26.42    26.38    12.32    12.31
60021045002     150.43   2.58    22.91    22.89     8.22     8.23
60021042002     150.40   2.26    25.53    25.81    12.14    12.14
60021031001     150.29   2.42    26.31    26.27    12.17    12.06
60021028001     150.16   2.11    24.56    24.54    11.13    11.13
60021092001     149.68   1.72    25.68    25.72    12.12    12.10
60021110001     150.60   2.18    23.82    23.68    11.22    11.20
60022011002     53.17   -27.74    44.79    44.78     7.04     6.94
60021039001     150.38   1.93    25.18    25.54    11.68    11.67
60021101002     150.65   1.64    26.24    26.29    12.61    12.59
60021083001     149.65   2.60    24.80    24.73    10.30    10.27
60022005001     52.92   -27.87    46.02    45.96    20.40    20.38
60021013001     149.97   2.46    26.55    26.61    10.36    10.25
60022002001     53.03   -27.98    45.92    45.98    21.65    21.59
60111043001     34.25   -4.80    50.19    50.36    23.69    23.68
60021019001     150.07   2.45    29.03    29.21    13.17    13.16
60021109001     150.69   2.07    25.10    25.02    12.47    12.47
60111006001     34.23   -5.23    50.57    50.46    13.62    13.60
60021072001     150.22   2.77    26.65    26.60    11.84    11.82
60021073001     150.08   2.68    25.95    25.89    11.29    11.26
60022011001     53.17   -27.75    47.76    47.72    21.86    21.84
60021119001     150.74   2.64    26.56    26.51    12.93    12.91
60023004004     214.83   52.79    51.28    51.20     2.69     2.69
60021041001     150.39   2.15    24.96    24.93    10.44    10.44
60021095001     150.01   1.69    26.55    26.88    12.40    12.38
60021049002     150.51   2.25    25.24    25.29    12.59    12.66
60111031002     34.64   -5.23    50.33    50.01    22.79    22.63
60021078001     149.87   2.79    26.87    26.80    12.25    12.32
60023004001     214.83   52.79    47.86    48.10     5.19     5.18
60023004002     214.81   52.81    46.73    46.51    21.59    21.63
60023004003     214.80   52.79    49.88    49.70     7.34     7.43
60022005002     52.93   -27.84    45.04    45.11     5.05     5.05
60022007002     53.17   -27.87    47.19    47.54    21.91    21.89
60022007003     53.18   -27.85    45.66    45.65     5.40     5.49
60111002002     34.16   -5.28    48.10    48.53    16.13    16.25
60021076001     150.00   2.78    24.82    24.66    10.72    10.69
60021017001     149.93   2.03    25.44    25.40    10.19    10.17
60021108001     150.59   2.08    28.41    28.35    14.04    13.92
60021115001     150.71   2.42    26.26    26.31    12.78    12.85
60021036002     150.28   1.94    24.45    24.44    10.77    10.76
60021066001     150.42   2.64    25.47    25.43    10.42    10.31
60022010001     53.04   -27.75    47.39    47.36    21.59    21.67
60022010004     53.06   -27.73    14.92    14.90     1.55     1.55
60022008001     53.29   -27.86    47.39    47.65    21.90    21.88
60022008002     53.30   -27.85    45.70    45.60     5.62     5.71
60022009001     52.92   -27.75    46.43    46.41    20.73    20.80
60021082001     149.65   2.70    27.49    27.44    12.15    12.14
60111018001     34.51   -5.24    49.28    49.44     7.37     7.44
60021044002     150.42   2.48    23.16    23.15    10.05    10.06
60021032001     150.28   2.31    26.71    26.78    12.29    12.28
60021081002     149.67   2.81    24.30    24.62    10.07    10.04
60111038001     34.74   -4.83    50.85    50.64    24.31    24.25
60022001003     52.92   -27.95    44.71    44.68     4.87     4.86
60021105001     150.67   1.86    26.25    26.21    12.66    12.65
60021027002     150.17   2.22    25.61    25.58    11.42    11.59
60111005002     34.21   -5.36    51.01    51.06    13.99    14.13
60021038001     150.37   1.83    24.64    24.73    10.15    10.25
60021048002     150.51   2.36    25.53    25.41    12.63    12.69
60021070001     150.33   2.75    25.22    25.15    11.46    11.43
60021085001     149.63   2.38    27.41    27.35    12.10    12.07
60021021001     150.05   2.24    27.75    27.74    12.29    12.28
60021074002     150.10   2.78    25.51    25.47     9.57     9.35
60021058001     149.89   2.63    23.02    22.84     7.52     7.60
60022004002     53.31   -27.95    44.72    44.95     5.20     5.04
60021059001     149.78   2.64    24.01    23.98     8.64     8.63
60021040001     150.38   2.05    23.86    24.02    11.47    11.46
60021064001     149.72   1.88    24.91    24.90     7.75     7.75
60023003005     214.72   52.71    52.26    52.28     3.23     3.24
60021037002     150.26   1.84    22.95    23.09    12.64    12.62
60023003001     214.72   52.71    48.21    48.12     4.76     4.75
60021086001     149.62   2.27    25.34    25.45    10.83    10.89
60023003002     214.70   52.74    46.47    46.24    21.74    21.69
60022012002     53.30   -27.74    46.04    46.02     7.38     7.47
60022012001     53.29   -27.75    47.99    48.14    22.02    22.11
60111010001     34.32   -5.01    47.36    47.54    10.82    10.70
60021114002     150.60   2.43    27.10    27.05    12.81    12.89
60021051001     150.49   2.03    22.03    22.10     8.77     8.77
60111004001     34.18   -5.00    49.64    49.69    15.08    15.14
60022013001     52.92   -27.64    48.50    48.41    22.10    22.19
60021060001     150.15   1.85    22.87    22.88     7.24     7.26
60022013002     52.93   -27.63    44.78    44.95     7.74     7.64
60023007001     215.15   53.01    50.40    50.36     7.78     7.77
60021022001     150.05   2.12    24.87    25.04    10.42    10.40
60023007005     215.10   53.01    48.64    48.67     5.76     5.94
60022003001     53.16   -27.98    45.90    45.95    21.56    21.54
60022003002     53.18   -27.95    44.90    44.86     5.32     5.22

